Trojans in Large Language Models of Code: A Critical Review through a Trigger-Based Taxonomy

Large language models (LLMs) have provided a lot of exciting new capabilities in software development. However, the opaque nature of these models makes them difficult to reason about and inspect. Their opacity gives rise to potential security risks, as adversaries can train and deploy compromised models to disrupt the software development process in the victims' organization. This work presents an overview of the current state-of-the-art trojan attacks on large language models of code, with a focus on triggers -- the main design point of trojans -- with the aid of a novel unifying trigger taxonomy framework. We also aim to provide a uniform definition of the fundamental concepts in the area of trojans in Code LLMs. Finally, we draw implications of findings on how code models learn on trigger design.

==> packages.tex <==

\usepackage{comment}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{cleveref}



\begin{comment}
\usepackage{geometry}
\usepackage{amsmath}
\usepackage{comment}
\usepackage{geometry}
\usepackage{pbox}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{float}
\usepackage{listings}
\usepackage{url} 
\usepackage{adjustbox}
\usepackage{microtype}
\usepackage{balance}
\usepackage{paralist}
\usepackage{fancyvrb}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{soul}
\usepackage{array}
\usepackage{listings}
%\usepackage{natbib}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\usepackage{multirow}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks

\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{fancyhdr}       % header
\usepackage{xcolor}
\graphicspath{{media/}}     % organize your images and other figures under media/ folder



%% For including figures, graphicx.sty has been loaded in
%% elsarticle.cls. If you prefer to use the old commands
%% please give \usepackage{epsfig}

%% The amssymb package provides various useful mathematical symbols
\usepackage{lipsum}

\usepackage{colortbl}
\definecolor{timberwolf}{rgb}{0.86, 0.84, 0.82}

% \usepackage{cite} % \bibliographystyle{IEEEtranS}
%\usepackage[numbers]{natbib} % \bibliographystyle{IEEEtranN}

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{todonotes}
\usepackage{textcomp}
 \usepackage{multirow}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{comment}
\usepackage{cleveref}  % Cref
\usepackage{xspace}

% bowen comment
\usepackage{xcolor}
\usepackage{enumitem}
\newcommand{\basicalert}[2]{\fbox{\bfseries\sffamily\scriptsize\color{blue} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}
\newcommand{\bowen}[1]{\basicalert{From Bowen}{#1}}
%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
%% \usepackage{lineno}

%% You might want to define your own abbreviated commands for common used terms, e.g.:
\newcommand{\kms}{km\,s$^{-1}$}
\newcommand{\msun}{$M_\odot}

\end{comment}

